Don't Memorize; Mimic The Past: Federated Class Incremental Learning Without Episodic Memory

Deep learning models are prone to forgetting information learned in the past when trained on new data. This problem becomes even more pronounced in the context of federated learning (FL), where data is decentralized and subject to independent changes for each user. Continual Learning (CL) studies this so-called \textit{catastrophic forgetting} phenomenon primarily in centralized settings, where the learner has direct access to the complete training dataset. However, applying CL techniques to FL is not straightforward due to privacy concerns and resource limitations. This paper presents a framework for federated class incremental learning that utilizes a generative model to synthesize samples from past distributions instead of storing part of past data. Then, clients can leverage the generative model to mitigate catastrophic forgetting locally. The generative model is trained on the server using data-free methods at the end of each task without requesting data from clients. Therefore, it reduces the risk of data leakage as opposed to training it on the client's private data. We demonstrate significant improvements for the CIFAR-100 dataset compared to existing baselines.

==> text/super.tex <==
\section{SuperImageNet}

In centralized Class-IL, the tasks are disjoint, and each task reveals a new set of classes; therefore, the total number of classes in the training dataset strongly limits the number of tasks. Moreover, we must ensure that each task has sufficient training data for learning. Thus, the number of examples per class is an important factor in creating CL datasets. 

\begin{table}
% \begin{table}[h]
	% \tiny\addtolength{\tabcolsep}{-3.5pt}
		\caption{Versions of SuperImageNet}
		\label{table:superimagenet}
		\centering
 		% \begin{adjustbox}{width=.85\linewidth}
        \small
		\begin{tabular}{ccc}
			% \hline
			% \rule{0pt}{3ex}
			\textbf{Dataset} & \textbf{\# examples/class} & \textbf{\# classes} \\
			\hline
                \hline
			\textit{SuperImageNet-S} & $2500$ & $100$\\
			% \hline
			\textit{SuperImageNet-M} & $5000$ & $75$ \\
			% \hline
			\textit{SuperImageNet-L} & $7500$ & $50$\\
			% \hline

		\end{tabular}
		% \end{adjustbox}
% 		\vspace{-4mm}
% \end{table} 
\end{table}
However, in a Federated class-IL setup, the dataset needs to be split along the task dimension and clients. For instance, CIFAR-100, a popular dataset for benchmarking FL algorithms, consists of $100$ classes, each with $500$ examples, must first be partitioned into $t$ tasks, and each task's data is split among $N$ clients. In other words, for a single task, a client has access to only $\frac{1}{t \times N}$ of that dataset. In a common scenario where $N=100$ and $t=10$, we can assign only $50$ samples to each client (about $5$ example per class in IID data distribution), which is hardly enough.

To resolve this problem, prior works have used a small $N$ \cite{qi2023better,hendryx2021federated,usmanova2021distillation}, combined multiple datasets \cite{yoon2021federated}, employed a surrogate dataset \cite{macontinual} or allowed data sharing among the clients \cite{dong2022federated}. However, these solutions may not be available, applicable, or may violate the FL's original assumptions. This clearly demonstrates how important it is to introduce new benchmark datasets for federated continual settings that can be efficiently split between both tasks and clients.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figs/sup.pdf}
\vspace{-5mm}
  \caption{Building SuperImageNet out of ImageNet classes. Yellow: labels in ImageNet, Red: label in SuperImageNet.}
  \label{fig:sup}
  \vspace{-2mm}
\end{figure}
We introduce \textbf{SuperImageNet}, a dataset created by superclassing the \textit{ImageNet}\cite{deng2009imagenet} dataset, thus greatly increasing the number of available samples for each class. We release $3$ versions of the dataset, each offering a different trade-off between the number of classes (for Class-IL) and the number of examples per class (for FL) as shown in Table \ref{table:superimagenet}. As an example, \textit{SuperImageNet-M} has \textit{10x} more examples per class compared to CIFAR-100, which allows for an order of magnitude increase in the number of clients in a federated setting while maintaining the same amount of training data per client. As shown in Fig. \ref{fig:sup}, to increase the sample size per class, we have merged classes of similar concepts. %In other words, as we move from ImageNet to SuperImageNet-S to SuperImageNet-L, class sizes increase, and each class represents a more general entity.
% \vspace{-4mm}
